How do information security workers use host data? A summary of interviews with security analysts

Modern security operations centers (SOCs) employ a variety of tools for intrusion detection, prevention, and widespread log aggregation and analysis. While research efforts are quickly proposing novel algorithms and technologies for cyber security, access to actual security personnel, their data, and their problems are necessarily limited by security concerns and time constraints. To help bridge the gap between researchers and security centers, this paper reports results of semi-structured interviews of 13 professionals from five different SOCs including at least one large academic, research, and government organization. The interviews focused on the current practices and future desires of SOC operators about host-based data collection capabilities, what is learned from the data, what tools are used, and how tools are evaluated. Questions and the responses are organized and reported by topic. Then broader themes are discussed. Forest-level takeaways from the interviews center on problems stemming from size of data, correlation of heterogeneous but related data sources, signal-to-noise ratio of data, and analysts' time.

==> 431-tools-table.tex <==
\begin{table*}
\begin{threeparttable}
\caption{Host Data \& Detection Products Reported}
\label{tab:tools}
\begin{tabular}{p{.5cm} p{4cm} p{5.7cm} p{7cm} }
\toprule
& \multicolumn{1}{c}{\textbf{Product}} & \multicolumn{1}{c}{\textbf{Description}}         & \multicolumn{1}{c}{\textbf{URL}}    
\\
\midrule
\parbox[c]{4mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Data}}}}\parbox[c]{4mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Store}}}} & Splunk                               & Log collection, SIEM, other    & \url{www.splunk.com}\\
&Snare                                & Log collection,  SIEM, other    & \url{www.snaresolutions.com}                                                         \\
&ElasticSearch                        & Open source database, other          & \url{www.elastic.co}                                                                 \\
& Log Insight  & Log management & \url{www.vmware.com}\\
\midrule

\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Host \phantom{Aa}}}}}\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Configuration}}}} 
& IBM BigFix                           & Endpoint management \& configuration             & \url{www.ibm.com/security/endpoint-security/bigfix}                                  \\ 
&Microsoft Sysmon                     & Endpoint logging configuration                   & \url{https://docs.microsoft.com/en-us/sysinternals/downloads/sysmon}                 \\
& WLS                                 & Windows Logging Service  & \url{https://digirati82.com/wls-information/}\\
& JAMF & Mac management \& configuration & \url{www.jamf.com}\\

\midrule

\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\phantom{llla}}}}\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Endpoint AV \phantom{llla}}}}}
& McAfee                               & Endpoint AV                                      & \url{www.mcafee.com}                                                                 \\
& Sophos                               & Endpoint AV                                      & \url{www.sophos.com}                                                                 \\
& Windows Defender           & Endpoint AV for Windows                          & \url{www.microsoft.com/en-us/windows/windows-defender}                               \\
& ESET                                 & Endpoint AV for Macs                             & \url{www.eset.com}                                                                   \\
& Sourcefire AMP                       & Endpoint AV                                      & \url{www.cisco.com/c/en/us/products/security/advanced-malware-protection/index.html} \\
& Carbon Black                         & Endpoint AV, application blacklisting            & \url{www.carbonblack.com}                                                            \\
& Symantic Endpoint Security           & Endpoint AV                                      & \url{www.symantec.com/products/endpoint}                                             \\
& Cylance                               & AI-based endpoint AV                              & \url{www.cylance.com}\\

\midrule 
\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\phantom{llla}}}}\parbox[c]{4mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Other \phantom{lll}}}}}
&Tenable Security Center      & Asset \& vulnerability scanning & \url{www.tenable.com}\\
& Flexera (Secunia) & Vulnerability management & \url{www.flexera.com/products/software-vulnerability-management}\\
& Qualys & Vulnerability management & \url{www.qualys.com/} \\
& Spirion                              & Data loss prevention, PII finder, other          & \url{www.spirion.com}                                                                \\
& EnCase                               & Forensic imaging toolsuite                       & \url{www.guidancesoftware.com/encase-forensic} \\                                     
& Cisco Email Security                 & Email security management                        & \url{www.cisco.com/c/en/us/products/security/email-security/index.html}              \\
& SCOT & Ticketing system & \url{https://github.com/sandialabs/scot}\\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

